NEVIS'22: A Stream of 100 Tasks Sampled from 30 Years of Computer Vision Research

A shared goal of several machine learning communities like continual learning, meta-learning and transfer learning, is to design algorithms and models that efficiently and robustly adapt to unseen tasks. An even more ambitious goal is to build models that never stop adapting, and that become increasingly more efficient through time by suitably transferring the accrued knowledge. Beyond the study of the actual learning algorithm and model architecture, there are several hurdles towards our quest to build such models, such as the choice of learning protocol, metric of success and data needed to validate research hypotheses. In this work, we introduce the Never-Ending VIsual-classification Stream (NEVIS'22), a benchmark consisting of a stream of over 100 visual classification tasks, sorted chronologically and extracted from papers sampled uniformly from computer vision proceedings spanning the last three decades. The resulting stream reflects what the research community thought was meaningful at any point in time, and it serves as an ideal test bed to assess how well models can adapt to new tasks, and do so better and more efficiently as time goes by. Despite being limited to classification, the resulting stream has a rich diversity of tasks from OCR, to texture analysis, scene recognition, and so forth. The diversity is also reflected in the wide range of dataset sizes, spanning over four orders of magnitude. Overall, NEVIS'22 poses an unprecedented challenge for current sequential learning approaches due to the scale and diversity of tasks, yet with a low entry barrier as it is limited to a single modality and well understood supervised learning problems. Moreover, we provide a reference implementation including strong baselines and an evaluation protocol to compare methods in terms of their trade-off between accuracy and compute.

==> cover_letter_resubmission.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editor:

We thank the reviewers and you for the valuable feedback. We are writing to re-submit our manuscript ``\red{NEVIS'22: A Stream of 100 Tasks Sampled from 30 Years of Computer Vision Research}'' to the \emph{Journal of Machine Learning Research}. We have thoroughly revised the paper to address all the points raised by the reviewers. In this revised version, we have marked in red the changes that we have made. Obviously, we will remove these markings once the paper is accepted.

As already mentioned, this paper \red{does not extend any prior work}.

We suggest the following referees for our submission.

Reviewers from the JMLR list:
\begin{itemize}
    \item \red{Joaquin Vanschoren, Eindhoven University of Technology (j.vanschoren@tue.nl)}
    \item \red{Cedric Archambeau, Amazon (cedrica@amazon.com)}
    \item \red{Hao Li, Amazon (haoli@cs.umd.edu)}
    \item \red{Marius Lindauer, Leibniz University Hannover (lindauer@tnt.uni-hannover.de)}
    \item \red{Jan N. van Rijn, University of Leiden (
j.n.van.rijn@liacs.leidenuniv.nl)}
\end{itemize}
Reviewers with competence in Continual Learning (missing from the official JMLR list):
\begin{itemize}
    \item \red{Christopher Kanan, University of Rochester (chriskanan@gmail.com)}
    \item \red{Tyler L. Hayes, Naver Labs (tlh6792@rit.edu)}
    \item \red{Diane Larlus, Naver Labs (diane.larlus@naverlabs.com )}
    \item \red{Karteek Alahari, Inria (karteek.alahari@inria.fr)}
    \item \red {Zeynep Akata, University of Tubingen (zeynep.akata@uni-tuebingen.de)}
\end{itemize}




Our submission has the following keywords: 
\red{benchmark}, \red{transfer learning}, \red{continual learning}, \red{meta-learning},  \red{AutoML}.

As the corresponding author and to the best of my knowledge, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip
J\"org Bornschein \\
Alexandre Galashov\\
Ross Hemsley\\
Amal Rannen-Triki\\
Yutian Chen \\
Arslan Chaudhry \\
Xu Owen He \\
Arthur Douillard \\ 
Massimo Caccia\\ 
Qixuan Feng \\
Jiajun Shen\\ 
Sylvestre-Alvise Rebuffi\\ 
Kitty Stacpoole\\ 
Diego de las Casas\\ 
Will Hawkins\\
Angeliki Lazaridou\\ 
Yee Whye Teh\\ 
Andrei A. Rusu\\ 
Razvan Pascanu\\
Marc’Aurelio Ranzato \\
All co-authors from DeepMind. Massimo Caccia is currently affiliated to University of Montreal but the work was done during his internship at DeepMind.

\end{document}







































